Revealing Neural Network Bias to Non-Experts Through Interactive Counterfactual Examples

AI algorithms are not immune to biases. Traditionally, non-experts have little control in uncovering potential social bias (e.g., gender bias) in the algorithms that may impact their lives. We present a preliminary design for an interactive visualization tool CEB to reveal biases in a commonly used AI method, Neural Networks (NN). CEB combines counterfactual examples and abstraction of an NN decision process to empower non-experts to detect bias. This paper presents the design of CEB and initial findings of an expert panel (n=6) with AI, HCI, and Social science experts.

==> wachter_notes.tex <==

". Grgic-Hlaca et al.
59 showed how
understandable models can easily mislead our intuitions, and that
predominantly using features people believed to be fair slightly increased
the racism exhibited by algorithms, while decreasing accuracy. In general,
the best tools for uncovering systematic biases are likely to be based upon
large-scale statistical analysis and not upon explanations of individual
decisions.60"


56 See Kilbertus et al., supra note 54, at 1.
57 See Matt J. Kusner et al., Counterfactual Fairness, AʀXɪᴠ:1703.06856, at 16 (2017),
https://arxiv.org/pdf/1703.06856.pdf [https://perma.cc/4SVN-7J9D].
58 Id.
59 Nina Grgic-Hlaca et al., The Case for Process Fairness in Learning: Feature Selection
for Fair Decision Making, in NIPS SYMPOSIUM ON MACHINE LEARNING AND THE LAW
8 (2016).
60 See Andrea Romei & Salvatore Ruggieri, A Multidisciplinary Survey on
Discrimination Analysis, 29 KNOWLEDGE ENGINEERING REV. 582, 617 (2014).
61 Establishing the influence of a protected variable on a decision does not, by itself,
prove that illegal discrimination has occurred. Mitigating factors may exist which justify
the usage of a protected attribute. See, e.g., Solon Barocas & Andrew D. Selbst, Big
Data’s Disparate Impact, 104 CAL. L. REV. 671, 676 (2016) (discussing disparate
treatment in American anti-discrimination law).


Several works have approached the problem of guaranteeing that
algorithms are fair, i.e. that they do not exhibit a bias towards particular
ethnic, gender, or other protected groups, using causal reasoning56 and
counterfactuals.
57 Kusner et al.58 consider counterfactuals where the
subject belongs to a different race or sex, and require that the decision
made remain the same under such a counterfactual for it to be considered
fair. In contrast, we consider counterfactuals in which the decision differs
from its current state.
Many works have suggested that transparency might be a useful
tool for enforcing fairness. While it is unclear how counterfactuals could
be used for this purpose, it is also unclear if any form of explanation of
individual decisions can in fact help. Grgic-Hlaca et al.
59 showed how
understandable models can easily mislead our intuitions, and that
predominantly using features people believed to be fair slightly increased
the racism exhibited by algorithms, while decreasing accuracy. In general,
the best tools for uncovering systematic biases are likely to be based upon
large-scale statistical analysis and not upon explanations of individual
decisions.60
With that said, counterfactuals can provide evidence that an
algorithmic decision is affected by a protected variable (e.g. race), and
that it may therefore be discriminatory.
61 For the types of distance
function we consider in the next section, if the counterfactuals found
change someone’s race, then the treatment of that individual is dependent
on race. However, the converse statement is not true. Counterfactuals
which do not modify a protected attribute cannot be used as evidence that
the attribute was irrelevant to the decision. This is because counterfactuals
describe only some of the dependencies between a particular decision and

56 See Kilbertus et al., supra note 54, at 1.
57 See Matt J. Kusner et al., Counterfactual Fairness, AʀXɪᴠ:1703.06856, at 16 (2017),
https://arxiv.org/pdf/1703.06856.pdf [https://perma.cc/4SVN-7J9D].
58 Id.
59 Nina Grgic-Hlaca et al., The Case for Process Fairness in Learning: Feature Selection
for Fair Decision Making, in NIPS SYMPOSIUM ON MACHINE LEARNING AND THE LAW
8 (2016).
60 See Andrea Romei & Salvatore Ruggieri, A Multidisciplinary Survey on
Discrimination Analysis, 29 KNOWLEDGE ENGINEERING REV. 582, 617 (2014).
61 Establishing the influence of a protected variable on a decision does not, by itself,
prove that illegal discrimination has occurred. Mitigating factors may exist which justify
the usage of a protected attribute. See, e.g., Solon Barocas & Andrew D. Selbst, Big
Data’s Disparate Impact, 104 CAL. L. REV. 6
